Kings of the Milky Way: A Homogeneous Gaia DR3 Analysis of King Open Clusters and the Galactic Disc Metallicity Gradient

This study aims to establish an internally homogeneous set of structural, astrophysical, and kinematical parameters for King open clusters and to assess their role as tracers of the Galactic thin disc. We present a homogeneous structural, astrophysical, and kinematical analysis of 27 King open clusters using high-precision Gaia DR3 astrometry, photometry, and spectroscopy. Cluster reddenings, distances, metallicities, and ages are determined via a homogeneous Markov Chain Monte Carlo isochrone-fitting approach applied to Gaia colour-magnitude diagrams. The derived parameters span E(G_BP-G_RP) = 0.113-1.933 mag, metallicities of [Fe/H] = -0.40 to +0.28 dex, ages from 17 to 6166 Myr, and heliocentric distances between 739 and 6272 pc. A comparison between astrometric and isochrone-based distances yields a median parallax difference of $-13\mu$as, indicating a good level of internal consistency between the photometric and astrometric distance scales within the adopted homogeneous framework. The radial metallicity behaviour of the King clusters is also examined using three complementary Galactic distance definitions and compared with the metallicity-radius relations obtained independently from 164 spectroscopically analysed open clusters from the literature. The King-cluster gradients are close to $-0.060$ dex kpc$^{-1}$ and are broadly consistent with those of the external reference sample, indicating that the homogeneously analysed King clusters follow the negative metallicity-radius trend traced by the broader thin-disc open-cluster population. Flatter gradients are found for young clusters, suggesting more homogeneous chemical enrichment at recent epochs. When dynamical constraints are applied to reduce the effects of radial migration and orbital blurring, the inferred gradient remains close to $-0.059$ dex kpc$^{-1}$.

==> CDS_table.tex <==
\begin{table*}
\setcounter{table}{1}
\setlength{\tabcolsep}{3pt}
%\renewcommand{\arraystretch}{1.5}
\footnotesize
  \centering
    \caption{Equatorial coordinates, $G$-band apparent magnitudes, radial velocities and their uncertainties, \texttt{RUWE} parameters, cluster membership probabilities, and survey program information for 403 cluster member stars identified in the {\it Gaia} DR3 and \citet{Tsantaki_2022} catalogues for 25 King OCs with available radial velocity data.}
    \begin{tabular}{clcccccccccl}
    \hline
ID        & Cluster & Order & Gaia Source ID              & RA       & DEC       & $G$    & $R_{\rm V}$     & $R_{{\rm V}_{\rm err}}$ & RUWE &  $P$ & Survey \\
          &         &       &                             & (degree) & (degree)  & (mag)  & (km s$^{-1})$ & (km s$^{-1})$   &      &      &       \\
\hline
    1     & King 01 & 1     & Gaia DR3 431163215575253120 & 6.097863 & 64.193112 & 15.097 & -26.94 & 9.80  & 0.989 & 0.980 & Gaia \\
    2     & King 01 & 2     & Gaia DR3 431165689476321536 & 6.038069 & 64.312581 & 14.903 & -49.86 & 4.31  & 1.022 & 0.992 & Gaia \\
    3     & King 01 & 3     & Gaia DR3 431166823347639424 & 5.828801 & 64.365959 & 14.273 & -52.62 & 1.99  & 1.052 & 0.996 & Gaia \\
    4     & King 01 & 4     & Gaia DR3 431167922859422208 & 5.648368 & 64.123386 & 13.143 & -53.57 & 1.30  & 1.059 & 0.986 & Gaia \\
    5     & King 01 & 5     & Gaia DR3 431171221394186496 & 5.517241 & 64.267695 & 15.315 & -52.65 & 5.87  & 1.018 & 0.998 & Gaia \\
    6     & King 01 & 6     & Gaia DR3 431173008102097664 & 5.265391 & 64.214066 & 10.817 & -53.22 & 0.15  & 1.098 & 0.971 & Gaia \\
    7     & King 01 & 7     & Gaia DR3 431173931509862656 & 5.391857 & 64.262292 & 12.401 & -52.61 & 0.24  & 1.064 & 0.994 & Gaia \\
    8     & King 01 & 8     & Gaia DR3 431174348130215808 & 5.369721 & 64.295763 & 15.089 & -53.21 & 3.67  & 1.092 & 0.998 & Gaia \\
    9     & King 01 & 9     & Gaia DR3 431176478434151808 & 5.754961 & 64.303916 & 15.003 & -49.33 & 5.64  & 1.010 & 0.998 & Gaia \\
    10    & King 01 & 10    & Gaia DR3 431176684592574208 & 5.706753 & 64.311387 & 14.362 & -53.83 & 2.06  & 1.083 & 0.999 & Gaia \\
    11    & King 01 & 11    & Gaia DR3 431176753312042368 & 5.686131 & 64.323678 & 15.188 & -51.33 & 5.96  & 1.027 & 0.996 & Gaia \\
    12    & King 01 & 12    & Gaia DR3 431177199988645760 & 5.562914 & 64.299549 & 15.302 & -61.30 & 4.37  & 1.256 & 0.998 & Gaia \\
    13    & King 01 & 13    & Gaia DR3 431177749744427392 & 5.553636 & 64.352826 & 14.977 & -72.71 & 9.44  & 1.163 & 0.999 & Gaia \\
    14    & King 01 & 14    & Gaia DR3 431177852823617664 & 5.504396 & 64.384233 & 15.276 &  6.49  & 6.73  & 0.979 & 0.994 & Gaia \\
    15    & King 01 & 15    & Gaia DR3 431177852823619584 & 5.514491 & 64.381705 & 14.963 & -44.43 & 17.44 & 1.127 & 0.999 & Gaia \\
    16    & King 01 & 16    & Gaia DR3 431177852823626368 & 5.529077 & 64.373030 & 13.421 & -53.74 & 1.91  & 1.055 & 0.999 & Gaia \\
    17    & King 01 & 17    & Gaia DR3 431179021054740352 & 5.628678 & 64.371613 & 15.278 & -31.26 & 5.59  & 1.033 & 0.999 & Gaia \\
    18    & King 01 & 18    & Gaia DR3 431179089774212096 & 5.593873 & 64.374980 & 15.274 & -53.05 & 5.75  & 1.058 & 0.999 & Gaia \\
    19    & King 01 & 19    & Gaia DR3 431179089774212480 & 5.587270 & 64.373212 & 13.578 & -52.29 & 0.84  & 1.077 & 0.999 & Gaia \\
    20    & King 01 & 20    & Gaia DR3 431179124133951360 & 5.640934 & 64.378948 & 14.985 & -68.99 & 7.76  & 0.999 & 0.999 & Gaia \\
    21    & King 01 & 21    & Gaia DR3 431179364652100224 & 5.537734 & 64.396300 & 12.644 & -52.72 & 0.42  & 1.127 & 0.996 & Gaia \\
    22    & King 01 & 22    & Gaia DR3 431179364652501248 & 5.526164 & 64.403370 & 15.131 & -67.90 & 6.15  & 1.018 & 0.998 & Gaia \\
    23    & King 01 & 23    & Gaia DR3 431179399011841920 & 5.573500 & 64.395713 & 15.084 & -60.82 & 8.09  & 1.087 & 1.000 & Gaia \\
    24    & King 01 & 24    & Gaia DR3 431179433371570560 & 5.575236 & 64.410813 & 12.333 & -53.81 & 0.27  & 1.011 & 0.999 & Gaia \\
    25    & King 01 & 25    & Gaia DR3 431179433371574784 & 5.587410 & 64.405754 & 15.126 & -36.81 & 5.93  & 1.105 & 0.999 & Gaia \\
    26    & King 01 & 26    & Gaia DR3 431179639529997184 & 5.616769 & 64.422634 & 15.174 & -46.27 & 6.61  & 1.076 & 0.999 & Gaia \\
    27    & King 01 & 27    & Gaia DR3 431179811328687616 & 5.567441 & 64.419062 & 15.167 & -67.70 & 7.07  & 1.019 & 0.999 & Gaia \\
    28    & King 01 & 28    & Gaia DR3 431179880048155008 & 5.521111 & 64.433158 & 14.883 & -49.23 & 5.64  & 1.034 & 0.999 & Gaia \\
    29    & King 01 & 29    & Gaia DR3 431180258005332864 & 5.484720 & 64.335619 & 13.066 & -52.43 & 0.77  & 1.079 & 0.940 & Gaia \\
    30    & King 01 & 30    & Gaia DR3 431180322422113280 & 5.441471 & 64.343848 & 13.447 & -55.80 & 1.15  & 1.088 & 0.999 & Gaia \\
    31    & King 01 & 31    & Gaia DR3 431180326724797696 & 5.426285 & 64.347954 & 15.268 & -47.37 & 6.41  & 1.116 & 0.999 & Gaia \\
    32    & King 01 & 32    & Gaia DR3 431180532883212800 & 5.389498 & 64.364787 & 13.232 & -53.83 & 0.59  & 1.158 & 0.998 & Gaia \\
    33    & King 01 & 33    & Gaia DR3 431180597299101952 & 5.344272 & 64.376976 & 13.056 & -53.31 & 0.85  & 1.054 & 0.999 & Gaia \\
    34    & King 01 & 34    & Gaia DR3 431180601602681088 & 5.353854 & 64.374035 & 13.378 & -53.67 & 1.23  & 0.999 & 0.994 & Gaia \\
    35    & King 01 & 35    & Gaia DR3 431180631659820032 & 5.461350 & 64.358715 & 13.138 & -52.27 & 0.44  & 1.077 & 0.999 & Gaia \\
    36    & King 01 & 36    & Gaia DR3 431180635962447104 & 5.483104 & 64.349645 & 14.882 & -53.16 & 7.94  & 1.024 & 0.999 & Gaia \\
    37    & King 01 & 37    & Gaia DR3 431180666019532544 & 5.491483 & 64.354113 & 13.296 & -53.04 & 1.98  & 1.034 & 0.999 & Gaia \\
    38    & King 01 & 38    & Gaia DR3 431180670322175872 & 5.473323 & 64.362034 & 13.487 & -52.14 & 0.75  & 1.146 & 0.998 & Gaia \\
    39    & King 01 & 39    & Gaia DR3 431180704681915136 & 5.452101 & 64.358126 & 13.617 & -63.37 & 2.59  & 1.204 & 0.999 & Gaia \\
    40    & King 01 & 40    & Gaia DR3 431180739041636864 & 5.430127 & 64.380369 & 14.819 & -51.32 & 5.19  & 1.071 & 0.999 & Gaia \\
    41    & King 01 & 41    & Gaia DR3 431180940896484992 & 5.395603 & 64.388358 & 13.214 & -53.99 & 0.67  & 0.990 & 0.999 & Gaia \\
    42    & King 01 & 42    & Gaia DR3 431180979559800960 & 5.379682 & 64.380444 & 13.752 & -51.78 & 1.10  & 1.061 & 0.998 & Gaia \\
    43    & King 01 & 43    & Gaia DR3 431181009617110528 & 5.382104 & 64.394686 & 12.382 & -53.91 & 0.42  & 1.094 & 0.998 & Gaia \\
    44    & King 01 & 44    & Gaia DR3 431181013919534592 & 5.381640 & 64.389500 & 14.985 & -42.43 & 7.59  & 1.037 & 0.999 & Gaia \\
    45    & King 01 & 45    & Gaia DR3 431181048279272192 & 5.408695 & 64.393803 & 13.098 & -51.94 & 0.75  & 1.054 & 0.990 & Gaia \\
    46    & King 01 & 46    & Gaia DR3 431181632394726656 & 5.260844 & 64.407139 & 13.728 & -53.98 & 1.27  & 1.043 & 0.995 & Gaia \\
    47    & King 01 & 47    & Gaia DR3 431181632394727552 & 5.257106 & 64.400019 & 14.968 & -49.72 & 7.03  & 1.037 & 0.998 & Gaia \\
    48    & King 01 & 48    & Gaia DR3 431182212208194816 & 5.228454 & 64.452940 & 13.061 & -54.70 & 0.72  & 1.058 & 0.997 & Gaia \\
    49    & King 01 & 49    & Gaia DR3 431182285229854336 & 5.475148 & 64.400819 & 14.826 & -49.60 & 3.83  & 1.109 & 0.998 & Gaia \\
    50    & King 01 & 50    & Gaia DR3 431182285229855616 & 5.484505 & 64.399187 & 14.271 & -52.57 & 5.44  & 1.023 & 0.999 & Gaia \\
    51    & King 01 & 51    & Gaia DR3 431182285229862144 & 5.493104 & 64.390110 & 13.467 & -53.37 & 1.14  & 1.041 & 0.999 & Gaia \\
    52    & King 01 & 52    & Gaia DR3 431182388309056128 & 5.434348 & 64.421106 & 13.396 & -53.42 & 0.77  & 1.056 & 0.999 & Gaia \\
    53    & King 01 & 53    & Gaia DR3 431182422668797056 & 5.497042 & 64.421918 & 14.698 & -54.53 & 2.60  & 1.118 & 0.999 & Gaia \\
    54    & King 01 & 54    & Gaia DR3 431182560107744640 & 5.401912 & 64.423926 & 15.156 & -56.29 & 5.23  & 0.991 & 0.999 & Gaia \\
    55    & King 01 & 55    & Gaia DR3 431182766266164864 & 5.359745 & 64.457517 & 13.381 & -53.75 & 1.02  & 1.048 & 0.999 & Gaia \\
    56    & King 01 & 56    & Gaia DR3 431183453460930688 & 5.288541 & 64.454109 & 14.380 & -53.11 & 1.78  & 1.150 & 0.997 & Gaia \\
    57    & King 01 & 57    & Gaia DR3 431183655315812224 & 5.249991 & 64.475337 & 11.870 & -53.49 & 0.19  & 1.024 & 0.997 & Gaia \\
    58    & King 01 & 58    & Gaia DR3 431189706934379904 & 6.055609 & 64.366907 & 14.554 & -56.13 & 2.85  & 0.963 & 0.991 & Gaia \\
    59    & King 01 & 59    & Gaia DR3 431190600287538816 & 5.924220 & 64.414342 & 15.192 & -48.38 & 6.13  & 1.029 & 0.996 & Gaia \\
    60    & King 01 & 60    & Gaia DR3 431202248238830592 & 5.829503 & 64.423419 & 13.365 & -54.50 & 1.09  & 1.033 & 0.998 & Gaia \\
    61    & King 01 & 61    & Gaia DR3 431203588268558592 & 5.600551 & 64.482733 & 14.753 & -47.74 & 4.03  & 1.345 & 0.999 & Gaia \\
    62    & King 01 & 62    & Gaia DR3 431203966225634944 & 5.645809 & 64.536327 & 14.816 & -49.40 & 5.61  & 1.033 & 0.998 & Gaia \\
    63    & King 01 & 63    & Gaia DR3 431205718572245120 & 5.551278 & 64.578709 & 14.727 & -49.11 & 3.49  & 1.040 & 0.994 & Gaia \\
    64    & King 01 & 64    & Gaia DR3 431207196040989184 & 5.508410 & 64.580250 & 13.182 & -53.36 & 0.81  & 1.021 & 0.996 & Gaia \\
    65    & King 01 & 65    & Gaia DR3 431925623808254848 & 5.107965 & 64.314126 & 13.172 & -52.91 & 0.45  & 1.057 & 0.995 & Gaia \\
    66    & King 01 & 66    & Gaia DR3 431928716184657408 & 4.768422 & 64.395875 & 15.033 & -52.55 & 5.09  & 0.944 & 0.970 & Gaia \\
    67    & King 01 & 67    & Gaia DR3 431935553772495872 & 4.982748 & 64.567693 & 15.114 & -52.93 & 6.30  & 1.022 & 0.986 & Gaia \\
    68    & King 02 & 1     & Gaia DR3 424416887106024192 & 12.753033 & 58.182267 & 13.603 & -134.67 & 0.90  & 1.058 & 0.997 & Gaia \\
    69    & King 02 & 2     & Gaia DR3 424417024545008128 & 12.653210 & 58.144950 & 15.025 & -141.23 & 3.44  & 0.990 & 0.991 & Gaia \\
    70    & King 02 & 3     & Gaia DR3 424417505581133312 & 12.582982 & 58.201409 & 14.000 & -42.41 & 1.53  & 1.027 & 0.981 & Gaia \\
    71    & King 02 & 4     & Gaia DR3 424418673812373376 & 12.816598 & 58.231321 & 14.807 & -142.55 & 3.02  & 1.011 & 0.991 & Gaia \\
    72    & King 02 & 5     & Gaia DR3 424419361007110144 & 12.695787 & 58.261595 & 14.669 & -143.07 & 2.23  & 1.005 & 0.991 & Gaia \\
    73    & King 02 & 6     & Gaia DR3 424419738964232576 & 12.710395 & 58.262362 & 14.562 & -145.04 & 3.01  & 1.073 & 0.991 & Gaia \\
    74    & King 02 & 7     & Gaia DR3 424424755486025600 & 12.814564 & 58.282763 & 15.036 & -68.41 & 3.22  & 1.037 & 0.906 & Gaia \\
    75    & King 02 & 8     & Gaia DR3 424426885789755776 & 12.867505 & 58.364064 & 14.044 & -55.49 & 1.19  & 1.020 & 0.500 & Gaia \\
    76    & King 02 & 9     & Gaia DR3 425167956626047616 & 12.547714 & 58.173687 & 15.203 & -66.99 & 4.97  & 1.046 & 0.954 & Gaia \\
    77    & King 02 & 10    & Gaia DR3 424417505581133312 & 12.582970 & 58.201406 & 14.017 & -42.69 & 0.10  & 1.027 & 0.981 & APOGEE \\
    78    & King 02 & 11    & Gaia DR3 424416887106024192 & 12.753020 & 58.182263 & 13.622 & -135.67 & 0.06  & 1.058 & 0.997 & APOGEE \\
    79    & King 03 & 1     & Gaia DR3 512961554924678144 & 24.092257 & 64.524848 & 14.124 & -44.54 & 1.54  & 1.018 & 0.999 & Gaia \\
    80    & King 03 & 2     & Gaia DR3 512961589284406016 & 24.128339 & 64.533333 & 13.858 & -41.75 & 1.80  & 1.041 & 0.999 & Gaia \\
    81    & King 03 & 3     & Gaia DR3 512961589284409472 & 24.121387 & 64.530954 & 13.965 & -43.73 & 2.06  & 1.048 & 1.000 & Gaia \\
    82    & King 03 & 4     & Gaia DR3 512961692363595648 & 24.119211 & 64.551690 & 13.189 & -45.99 & 0.70  & 1.045 & 0.998 & Gaia \\
    83    & King 03 & 5     & Gaia DR3 512966674525644544 & 24.297155 & 64.563082 & 14.328 & -42.55 & 1.62  & 1.093 & 0.991 & Gaia \\
    84    & King 03 & 6     & Gaia DR3 512971484889090432 & 23.917247 & 64.495157 & 14.247 & -44.84 & 2.13  & 1.000 & 0.994 & Gaia \\
    85    & King 03 & 7     & Gaia DR3 512972927998081536 & 24.076018 & 64.521590 & 13.567 & -43.66 & 0.64  & 1.031 & 0.999 & Gaia \\
    86    & King 03 & 8     & Gaia DR3 512973305955183232 & 24.076561 & 64.538841 & 14.784 & 28.79 & 7.65  & 0.973 & 1.000 & Gaia \\
    87    & King 04 & 1     & Gaia DR3 464250402368404608 & 39.010708 & 59.016837 & 12.186 & -45.23 & 0.80  & 1.293 & 0.874 & Gaia \\
    88    & King 05 & 1     & Gaia DR3 445990095511421824 & 48.611260 & 52.553500 & 14.320 & -44.63 & 2.33  & 1.041 & 0.990 & Gaia \\
    89    & King 05 & 2     & Gaia DR3 445992466335199232 & 48.684386 & 52.663807 & 14.685 & -64.18 & 5.70  & 1.118 & 0.998 & Gaia \\
    90    & King 05 & 3     & Gaia DR3 445992638131994240 & 48.692437 & 52.689295 & 13.948 & -41.36 & 2.02  & 1.063 & 0.999 & Gaia \\
    91    & King 05 & 4     & Gaia DR3 445992638131996544 & 48.682324 & 52.686660 & 12.155 & -44.54 & 0.36  & 1.177 & 0.993 & Gaia \\
    92    & King 05 & 5     & Gaia DR3 445992672493625856 & 48.704579 & 52.688165 & 14.528 & 26.64 & 6.91  & 1.010 & 0.999 & Gaia \\
    93    & King 05 & 6     & Gaia DR3 445993703283922816 & 48.538161 & 52.630892 & 14.066 & -37.18 & 1.60  & 1.148 & 0.828 & Gaia \\
    94    & King 05 & 7     & Gaia DR3 445995386911078784 & 48.578993 & 52.682505 & 13.890 & -44.14 & 1.57  & 1.093 & 0.998 & Gaia \\
    95    & King 05 & 8     & Gaia DR3 445995593069492992 & 48.674689 & 52.695325 & 13.319 & -43.60 & 2.72  & 1.160 & 0.999 & Gaia \\
    96    & King 05 & 9     & Gaia DR3 445995627429227520 & 48.690680 & 52.700017 & 12.591 & -42.40 & 0.61  & 1.184 & 0.998 & Gaia \\
    97    & King 05 & 10    & Gaia DR3 445995627431124736 & 48.684532 & 52.701965 & 14.562 & -26.03 & 7.35  & 0.989 & 0.996 & Gaia \\
    98    & King 05 & 11    & Gaia DR3 445995661788970496 & 48.660098 & 52.697334 & 14.220 & -40.65 & 2.28  & 1.118 & 0.999 & Gaia \\
    99    & King 05 & 12    & Gaia DR3 445995833587660416 & 48.616029 & 52.711317 & 13.785 & -44.54 & 1.51  & 1.034 & 0.992 & Gaia \\
    100   & King 05 & 13    & Gaia DR3 445995867947391488 & 48.647078 & 52.724146 & 14.266 & -49.03 & 4.59  & 1.103 & 0.999 & Gaia \\
    101   & King 05 & 14    & Gaia DR3 445995971026604672 & 48.646202 & 52.733159 & 13.689 & -40.97 & 1.58  & 1.117 & 0.990 & Gaia \\
    102   & King 05 & 15    & Gaia DR3 445996142825319552 & 48.567742 & 52.693467 & 14.068 & -42.14 & 1.51  & 1.047 & 0.998 & Gaia \\
    103   & King 05 & 16    & Gaia DR3 445997066238337920 & 48.606172 & 52.793220 & 12.064 & -43.43 & 0.23  & 1.090 & 0.990 & Gaia \\
    104   & King 05 & 17    & Gaia DR3 446085306345863552 & 48.849504 & 52.666422 & 14.259 & -41.71 & 2.97  & 1.066 & 0.996 & Gaia \\
    105   & King 05 & 18    & Gaia DR3 446086440218338176 & 48.727335 & 52.686596 & 14.974 & -57.34 & 8.45  & 1.097 & 0.999 & Gaia \\
    106   & King 05 & 19    & Gaia DR3 446088364362531968 & 48.881652 & 52.760892 & 14.676 & -8.10 & 8.09  & 1.071 & 0.984 & Gaia \\
    107   & King 05 & 20    & Gaia DR3 446089463874203904 & 48.698509 & 52.710620 & 13.320 & -43.55 & 0.70  & 1.080 & 0.997 & Gaia \\
    108   & King 05 & 21    & Gaia DR3 446089498233931392 & 48.714786 & 52.726928 & 13.508 & -43.01 & 1.29  & 1.117 & 0.993 & Gaia \\
    109   & King 05 & 22    & Gaia DR3 446089670032608256 & 48.721828 & 52.758665 & 13.787 & -43.59 & 1.30  & 1.086 & 0.996 & Gaia \\
    110   & King 05 & 23    & Gaia DR3 446090013629982592 & 48.760906 & 52.769929 & 14.019 & -42.80 & 1.62  & 1.064 & 0.997 & Gaia \\
    111   & King 05 & 24    & Gaia DR3 446280332221486976 & 48.603285 & 52.931931 & 14.939 & -25.19 & 6.51  & 1.025 & 0.604 & Gaia \\
    112   & King 05 & 25    & Gaia DR3 445993703283922816 & 48.538159 & 52.630888 & 14.087 & -42.51 & 0.15  & 1.148 & 0.828 & APOGEE \\
    113   & King 05 & 26    & Gaia DR3 445995833587660416 & 48.616028 & 52.711312 & 13.804 & -44.92 & 0.11  & 1.034 & 0.992 & APOGEE \\
    114   & King 05 & 27    & Gaia DR3 445997066238337920 & 48.606169 & 52.793214 & 12.086 & -43.46 & 0.02  & 1.090 & 0.990 & APOGEE \\
    115   & King 06 & 1     & Gaia DR3 448507186864643840 & 52.369523 & 56.273787 & 15.061 & 17.62 & 6.90  & 1.033 & 0.991 & Gaia \\
    116   & King 06 & 2     & Gaia DR3 448510828996909824 & 52.208612 & 56.319809 & 12.606 & -30.87 & 22.36 & 1.001 & 0.994 & Gaia \\
    117   & King 06 & 3     & Gaia DR3 448511344392974976 & 52.263059 & 56.344371 & 14.737 & -23.30 & 7.78  & 1.035 & 0.981 & Gaia \\
    118   & King 06 & 4     & Gaia DR3 448511894148794368 & 52.152706 & 56.352601 & 14.887 & -29.73 & 8.28  & 1.102 & 0.994 & Gaia \\
    119   & King 06 & 5     & Gaia DR3 448512546983811072 & 52.173934 & 56.397187 & 14.985 & -1.15 & 7.53  & 1.048 & 0.996 & Gaia \\
    120   & King 06 & 6     & Gaia DR3 448516017317436928 & 51.839575 & 56.277823 & 13.772 & -14.02 & 7.56  & 1.077 & 0.994 & Gaia \\
    121   & King 06 & 7     & Gaia DR3 448516635792731520 & 51.792422 & 56.269621 & 13.878 & -11.50 & 5.15  & 1.018 & 0.992 & Gaia \\
    122   & King 06 & 8     & Gaia DR3 448516803292532992 & 51.858634 & 56.295390 & 12.057 & -19.25 & 11.29 & 0.992 & 0.995 & Gaia \\
    123   & King 06 & 9     & Gaia DR3 448516807591410688 & 51.862104 & 56.305779 & 14.021 & -17.86 & 5.88  & 1.003 & 0.994 & Gaia \\
    124   & King 06 & 10    & Gaia DR3 448520106126284288 & 51.807665 & 56.355328 & 11.591 & -18.09 & 13.76 & 1.019 & 0.995 & Gaia \\
    125   & King 06 & 11    & Gaia DR3 448521274357199744 & 51.742623 & 56.411821 & 14.742 & -30.64 & 25.03 & 1.028 & 0.994 & Gaia \\
    126   & King 06 & 12    & Gaia DR3 448523232862467584 & 51.936993 & 56.362294 & 14.044 & -20.65 & 6.14  & 0.930 & 0.984 & Gaia \\
    127   & King 06 & 13    & Gaia DR3 448523572162589696 & 51.906470 & 56.406510 & 14.233 & -2.20 & 7.69  & 1.000 & 0.996 & Gaia \\
    128   & King 06 & 14    & Gaia DR3 448523610820113792 & 51.919317 & 56.414369 & 15.014 & -28.34 & 8.07  & 0.984 & 0.997 & Gaia \\
    129   & King 06 & 15    & Gaia DR3 448523679539048448 & 51.965660 & 56.423656 & 14.245 & -17.84 & 6.15  & 1.039 & 0.997 & Gaia \\
    130   & King 06 & 16    & Gaia DR3 448523748258520064 & 51.960917 & 56.444207 & 11.644 & -41.44 & 9.35  & 0.986 & 0.997 & Gaia \\
    131   & King 06 & 17    & Gaia DR3 448524194935121536 & 52.078374 & 56.401317 & 14.359 & -32.96 & 13.06 & 0.954 & 0.995 & Gaia \\
    132   & King 06 & 18    & Gaia DR3 448524465515806848 & 52.167342 & 56.428733 & 14.868 & -23.54 & 12.84 & 1.110 & 0.993 & Gaia \\
    133   & King 06 & 19    & Gaia DR3 448524916489624960 & 52.033998 & 56.424137 & 14.607 & -23.34 & 5.60  & 1.045 & 0.998 & Gaia \\
    134   & King 06 & 20    & Gaia DR3 448525157007793408 & 51.992269 & 56.435313 & 14.432 & -27.47 & 6.05  & 0.942 & 0.991 & Gaia \\
    135   & King 06 & 21    & Gaia DR3 448525706763595520 & 52.063206 & 56.475945 & 12.518 & -18.20 & 5.64  & 1.019 & 0.997 & Gaia \\
    136   & King 06 & 22    & Gaia DR3 448525844202542592 & 52.098542 & 56.508820 & 14.392 & -21.15 & 7.19  & 1.088 & 0.996 & Gaia \\
    137   & King 06 & 23    & Gaia DR3 448526119080491008 & 51.851047 & 56.382425 & 12.056 & -27.76 & 4.39  & 1.113 & 0.996 & Gaia \\
    138   & King 06 & 24    & Gaia DR3 448526290879001088 & 51.806105 & 56.400837 & 14.399 & -29.85 & 13.28 & 0.927 & 0.996 & Gaia \\
    139   & King 06 & 25    & Gaia DR3 448529211457465344 & 52.042781 & 56.568298 & 14.315 & -35.40 & 8.62  & 1.015 & 0.994 & Gaia \\
    140   & King 06 & 26    & Gaia DR3 448529864291929472 & 52.015962 & 56.565328 & 14.808 & -23.87 & 6.89  & 1.015 & 0.996 & Gaia \\
    141   & King 06 & 27    & Gaia DR3 448529928712584192 & 51.984445 & 56.575358 & 12.817 & -21.76 & 3.93  & 1.204 & 0.996 & Gaia \\
    142   & King 06 & 28    & Gaia DR3 448601882302556032 & 52.371547 & 56.327203 & 14.879 & -35.92 & 5.47  & 1.170 & 0.982 & Gaia \\
    143   & King 06 & 29    & Gaia DR3 448606623946439936 & 52.244471 & 56.453885 & 12.360 & -31.41 & 10.18 & 0.873 & 0.994 & Gaia \\
    144   & King 06 & 30    & Gaia DR3 448606727025651712 & 52.269261 & 56.468594 & 14.521 & -53.29 & 6.49  & 1.093 & 0.991 & Gaia \\
    145   & King 06 & 31    & Gaia DR3 448607998335943552 & 52.547759 & 56.525778 & 14.123 & -0.88 & 6.75  & 1.075 & 0.954 & Gaia \\
    146   & King 06 & 32    & Gaia DR3 448619680647005952 & 52.198278 & 56.551049 & 12.507 & -53.60 & 17.20 & 1.020 & 0.994 & Gaia \\
    147   & King 06 & 33    & Gaia DR3 448621020676778624 & 52.355133 & 56.611710 & 14.791 & -37.99 & 6.11  & 0.979 & 0.962 & Gaia \\
    148   & King 06 & 34    & Gaia DR3 448622631287562496 & 52.405029 & 56.699898 & 14.396 & -11.67 & 8.03  & 0.952 & 0.956 & Gaia \\
    149   & King 06 & 35    & Gaia DR3 448622807383201024 & 52.093650 & 56.556755 & 14.297 & -23.54 & 6.04  & 1.045 & 0.992 & Gaia \\
    150   & King 06 & 36    & Gaia DR3 448627205429664512 & 52.500431 & 56.665188 & 14.398 & -29.93 & 6.67  & 1.015 & 0.945 & Gaia \\
    151   & King 06 & 37    & Gaia DR3 449271931561050112 & 51.558555 & 56.417348 & 12.736 & -20.02 & 8.27  & 0.797 & 0.948 & Gaia \\
    152   & King 06 & 38    & Gaia DR3 449272103359171712 & 51.656996 & 56.437021 & 14.421 & -10.53 & 5.86  & 1.072 & 0.986 & Gaia \\
    153   & King 06 & 39    & Gaia DR3 449273099792142848 & 51.588686 & 56.461824 & 14.055 & -5.11 & 7.33  & 0.951 & 0.976 & Gaia \\
    154   & King 06 & 40    & Gaia DR3 449278700428899456 & 51.802695 & 56.527784 & 11.512 & -41.35 & 9.67  & 1.005 & 0.993 & Gaia \\
    155   & King 06 & 41    & Gaia DR3 449279108448699520 & 51.801236 & 56.581837 & 12.166 & -7.87 & 9.62  & 0.899 & 0.993 & Gaia \\
    156   & King 06 & 42    & Gaia DR3 449283029755913856 & 51.695322 & 56.621113 & 14.563 & -27.68 & 6.01  & 1.051 & 0.989 & Gaia \\
    157   & King 06 & 43    & Gaia DR3 448512065947486720 & 52.099400 & 56.364417 & 13.629 & -12.07 & 3.63  & 0.971 & 0.997 & LAMOST \\
    158   & King 06 & 44    & Gaia DR3448516017317436928  & 51.839604 & 56.277814 & 13.783 & -19.72 & 2.91  & 1.077 & 0.994 & LAMOST \\
    159   & King 06 & 45    & Gaia DR3448511000795603712  & 52.193566 & 56.317135 & 13.859 & -15.77 & 3.82  & 1.086 & 0.983 & LAMOST \\
    160   & King 06 & 46    & Gaia DR3448527012433502976  & 51.892473 & 56.478053 & 12.984 & -22.00 & 3.67  & 0.914 & 0.984 & LAMOST \\
    161   & King 06 & 47    & Gaia DR3448520209205315328  & 51.722702 & 56.344874 & 13.092 & -25.45 & 3.31  & 1.023 & 0.989 & LAMOST \\
    162   & King 06 & 48    & Gaia DR3448459392468599936  & 52.318220 & 56.180775 & 13.795 & -27.44 & 3.08  & 0.963 & 0.984 & LAMOST \\
    163   & King 06 & 49    & Gaia DR3449271931561050112  & 51.558582 & 56.417341 & 12.748 & -25.89 & 4.57  & 0.797 & 0.948 & LAMOST \\
    164   & King 07 & 1     & Gaia DR3 250920579366918016 & 59.802093 & 51.663297 & 12.747 & -10.44 & 0.59  & 1.202 & 0.990 & Gaia \\
    165   & King 07 & 2     & Gaia DR3 250921717537736448 & 59.783954 & 51.735478 & 13.751 & -10.83 & 1.12  & 1.130 & 0.998 & Gaia \\
    166   & King 07 & 3     & Gaia DR3 250926046864741760 & 59.713239 & 51.812811 & 13.879 & -9.83 & 0.87  & 1.126 & 0.998 & Gaia \\
    167   & King 07 & 4     & Gaia DR3 250927661772450304 & 59.841955 & 51.758771 & 13.825 & -9.19 & 1.05  & 1.185 & 0.999 & Gaia \\
    168   & King 07 & 5     & Gaia DR3 250930543692017536 & 59.789432 & 51.760526 & 13.241 & -7.76 & 0.83  & 1.090 & 0.997 & Gaia \\
    169   & King 07 & 6     & Gaia DR3 250930547990487168 & 59.792235 & 51.755376 & 12.732 & -9.63 & 0.35  & 1.106 & 0.998 & Gaia \\
    170   & King 07 & 7     & Gaia DR3 250930547990488832 & 59.784125 & 51.755994 & 12.827 & -9.59 & 1.25  & 1.132 & 0.996 & Gaia \\
    171   & King 07 & 8     & Gaia DR3 250930582350216192 & 59.813087 & 51.762521 & 13.853 & -9.89 & 1.46  & 1.071 & 0.999 & Gaia \\
    172   & King 07 & 9     & Gaia DR3 250930616709962240 & 59.780725 & 51.762478 & 12.782 & -10.12 & 0.72  & 1.101 & 0.997 & Gaia \\
    173   & King 07 & 10    & Gaia DR3 250930685429413248 & 59.822834 & 51.783723 & 12.826 & -10.76 & 0.41  & 1.156 & 0.998 & Gaia \\
    174   & King 07 & 11    & Gaia DR3 250930822868389632 & 59.768125 & 51.771392 & 15.133 & 382.57 & 7.82  & 1.043 & 0.999 & Gaia \\
    175   & King 07 & 12    & Gaia DR3 250930857228108928 & 59.780226 & 51.792879 & 15.097 & 40.75 & 6.45  & 1.048 & 0.999 & Gaia \\
    176   & King 07 & 13    & Gaia DR3 250930857228116224 & 59.772923 & 51.787829 & 15.096 & 129.13 & 20.79 & 1.048 & 0.998 & Gaia \\
    177   & King 07 & 14    & Gaia DR3 250930925947585792 & 59.771697 & 51.795991 & 14.638 & 100.56 & 7.00  & 1.184 & 0.984 & Gaia \\
    178   & King 07 & 15    & Gaia DR3 250930925948393088 & 59.768496 & 51.800081 & 13.021 & -10.59 & 0.49  & 1.204 & 0.999 & Gaia \\
    179   & King 07 & 16    & Gaia DR3 250931127806592640 & 59.867870 & 51.811800 & 12.907 & -10.51 & 0.33  & 1.121 & 0.993 & Gaia \\
    180   & King 07 & 17    & Gaia DR3 250932094178649472 & 59.783015 & 51.865281 & 13.661 & -7.50 & 0.80  & 1.152 & 0.996 & Gaia \\
    181   & King 07 & 18    & Gaia DR3 251675604558554624 & 59.486666 & 51.768646 & 13.602 & -10.11 & 0.55  & 1.106 & 0.598 & Gaia \\
    182   & King 07 & 19    & Gaia DR3 250920579366918016 & 59.802100 & 51.663292 & 12.769 & -10.34 & 0.83  & 1.202 & 0.990 & LAMOST \\
    183   & King 07 & 20    & Gaia DR3 250932094178649472 & 59.783023 & 51.865275 & 13.686 & -7.66 & 0.70  & 1.152 & 0.996 & LAMOST \\
    184   & King 07 & 21    & Gaia DR3 250926046864741760 & 59.713247 & 51.812806 & 13.907 & -10.59 & 0.04  & 1.126 & 0.998 & APOGEE \\
    185   & King 07 & 22    & Gaia DR3 250931127806592640 & 59.867876 & 51.811795 & 12.933 & -10.51 & 0.04  & 1.121 & 0.993 & APOGEE \\
    186   & King 07 & 23    & Gaia DR3 250930547990487168 & 59.792242 & 51.755371 & 12.757 & -10.19 & 0.04  & 1.106 & 0.998 & APOGEE \\
    187   & King 07 & 24    & Gaia DR3 250930685429413248 & 59.822841 & 51.783717 & 12.855 & -10.30 & 0.02  & 1.156 & 0.998 & APOGEE \\
    188   & King 07 & 25    & Gaia DR3 250930543692017536 & 59.789437 & 51.760520 & 13.269 & -6.74 & 0.03  & 1.090 & 0.997 & APOGEE \\
    189   & King 07 & 26    & Gaia DR3 250930547990488832 & 59.784132 & 51.755989 & 12.855 & -15.06 & 0.03  & 1.132 & 0.996 & APOGEE \\
    190   & King 07 & 27    & Gaia DR3 250930925948393088 & 59.768503 & 51.800076 & 13.047 & -10.58 & 0.04  & 1.204 & 0.999 & APOGEE \\
    191   & King 08 & 1     & Gaia DR3 3454321803949410688 & 87.318311 & 33.614989 & 14.665 & 0.52  & 3.10  & 0.933 & 0.999 & Gaia \\
    192   & King 08 & 2     & Gaia DR3 3454321803949410944 & 87.323355 & 33.610824 & 14.854 & -6.78 & 3.99  & 1.016 & 0.998 & Gaia \\
    193   & King 08 & 3     & Gaia DR3 3454321907028609920 & 87.322957 & 33.633610 & 15.267 & 24.10 & 9.62  & 1.058 & 0.999 & Gaia \\
    194   & King 08 & 4     & Gaia DR3 3454321907028614016 & 87.318284 & 33.632340 & 14.957 & -4.56 & 5.24  & 0.988 & 0.999 & Gaia \\
    195   & King 08 & 5     & Gaia DR3 3454322319345450752 & 87.339260 & 33.647835 & 14.828 & 0.34  & 4.77  & 0.964 & 0.999 & Gaia \\
    196   & King 09 & 1     & Gaia DR3 2005040512187406848 & 333.920879 & 54.401376 & 12.670 & -59.97 & 0.36  & 1.050 & 0.985 & Gaia \\
    197   & King 09 & 2     & Gaia DR3 2005040649614888064 & 333.875256 & 54.404708 & 15.400 & -61.21 & 11.59 & 1.192 & 0.986 & Gaia \\
    198   & King 09 & 3     & Gaia DR3 2005040683986088064 & 333.886117 & 54.400346 & 15.279 & -107.60 & 10.80 & 0.969 & 0.982 & Gaia \\
    199   & King 09 & 4     & Gaia DR3 2005040683986091136 & 333.899955 & 54.402640 & 15.220 & -57.97 & 5.08  & 0.955 & 0.985 & Gaia \\
    200   & King 09 & 5     & Gaia DR3 2005040752705552768 & 333.878667 & 54.411753 & 13.983 & -62.33 & 1.53  & 1.022 & 0.982 & Gaia \\
    201   & King 09 & 6     & Gaia DR3 2005040752705554048 & 333.878229 & 54.409117 & 14.283 & -57.36 & 1.98  & 0.994 & 0.986 & Gaia \\
    202   & King 09 & 7     & Gaia DR3 2005040752705560064 & 333.884122 & 54.404576 & 14.726 & -50.58 & 5.34  & 1.019 & 0.985 & Gaia \\
    203   & King 09 & 8     & Gaia DR3 2005791822225985280 & 333.738900 & 54.407969 & 14.558 & -48.98 & 3.70  & 0.998 & 0.589 & Gaia \\
    204   & King 09 & 9     & Gaia DR3 2005791822226143872 & 333.753282 & 54.416627 & 14.596 & -61.66 & 2.88  & 0.931 & 0.814 & Gaia \\
    205   & King 10 & 1     & Gaia DR3 2013491221110623104 & 343.741762 & 59.143433 & 14.709 & -127.23 & 6.72  & 1.208 & 0.998 & APOGEE \\
    206   & King 10 & 2     & Gaia DR3 2013491564707995776 & 343.766233 & 59.175533 & 14.666 & -83.70 & 6.73  & 0.980 & 0.999 & APOGEE \\
    207   & King 10 & 3     & Gaia DR3 2013494004249514752 & 343.636204 & 59.141852 & 10.055 & -62.74 & 0.20  & 0.950 & 0.955 & Gaia \\
    208   & King 10 & 4     & Gaia DR3 2013494549701474432 & 343.740350 & 59.195549 & 13.788 & -35.64 & 3.39  & 1.043 & 0.998 & APOGEE \\
    209   & King 11 & 1     & Gaia DR3 2211121972266402304 & 356.899500 & 68.559192 & 12.045 & -25.22 & 0.16  & 0.965 & 0.998 & Gaia \\
    210   & King 11 & 2     & Gaia DR3 2211122045287064320 & 356.806992 & 68.544132 & 15.256 & -24.03 & 4.13  & 1.042 & 0.997 & Gaia \\
    211   & King 11 & 3     & Gaia DR3 2211122045287373312 & 356.811594 & 68.547028 & 14.732 & -22.35 & 2.31  & 0.982 & 0.997 & Gaia \\
    212   & King 11 & 4     & Gaia DR3 2211122182726015232 & 356.885542 & 68.565103 & 14.856 & -22.26 & 4.30  & 0.969 & 0.998 & Gaia \\
    213   & King 11 & 5     & Gaia DR3 2211122251445487360 & 356.871186 & 68.571434 & 14.925 & -26.48 & 3.83  & 1.058 & 0.999 & Gaia \\
    214   & King 11 & 6     & Gaia DR3 2211125099003567744 & 356.744355 & 68.558868 & 14.636 & -22.25 & 2.51  & 1.060 & 0.997 & Gaia \\
    215   & King 11 & 7     & Gaia DR3 2211125275102455552 & 356.874928 & 68.591355 & 14.956 & -20.94 & 4.11  & 0.970 & 0.999 & Gaia \\
    216   & King 11 & 8     & Gaia DR3 2211125343821928448 & 356.787133 & 68.583735 & 13.740 & -25.69 & 1.17  & 0.912 & 0.999 & Gaia \\
    217   & King 11 & 9     & Gaia DR3 2211125412541398656 & 356.793434 & 68.597992 & 15.272 & -23.14 & 3.91  & 1.063 & 0.998 & Gaia \\
    218   & King 11 & 10    & Gaia DR3 2211125549980346240 & 356.901047 & 68.628098 & 14.913 & -21.78 & 3.55  & 1.009 & 1.000 & Gaia \\
    219   & King 11 & 11    & Gaia DR3 2211125549980348928 & 356.874441 & 68.618542 & 14.524 & -26.84 & 2.61  & 1.077 & 0.998 & Gaia \\
    220   & King 11 & 12    & Gaia DR3 2211125584340093952 & 356.532075 & 68.547264 & 15.055 & -24.64 & 3.67  & 0.980 & 0.987 & Gaia \\
    221   & King 11 & 13    & Gaia DR3 2211125790498515968 & 356.632176 & 68.581880 & 14.484 & -23.50 & 2.27  & 1.040 & 0.996 & Gaia \\
    222   & King 11 & 14    & Gaia DR3 2211126065376413952 & 356.650291 & 68.607438 & 15.292 & -24.61 & 5.06  & 1.039 & 0.997 & Gaia \\
    223   & King 11 & 15    & Gaia DR3 2211126168455636224 & 356.787656 & 68.611309 & 15.404 & -28.61 & 6.53  & 0.996 & 0.999 & Gaia \\
    224   & King 11 & 16    & Gaia DR3 2211126237175107328 & 356.774766 & 68.620259 & 14.135 & -23.46 & 1.36  & 1.105 & 0.999 & Gaia \\
    225   & King 11 & 17    & Gaia DR3 2211126237175108864 & 356.766701 & 68.616596 & 13.127 & -26.00 & 0.49  & 0.990 & 0.999 & Gaia \\
    226   & King 11 & 18    & Gaia DR3 2211126271534849664 & 356.849831 & 68.624655 & 15.039 & -25.23 & 3.11  & 0.993 & 0.999 & Gaia \\
    227   & King 11 & 19    & Gaia DR3 2211126305894587392 & 356.867390 & 68.629346 & 13.671 & -24.48 & 1.19  & 1.004 & 0.997 & Gaia \\
    228   & King 11 & 20    & Gaia DR3 2211126443333533824 & 356.789942 & 68.636061 & 15.320 & -36.13 & 4.21  & 0.926 & 0.999 & Gaia \\
    229   & King 11 & 21    & Gaia DR3 2211126615132221952 & 356.808082 & 68.651205 & 14.962 & -23.15 & 3.48  & 1.008 & 0.999 & Gaia \\
    230   & King 11 & 22    & Gaia DR3 2211203958901905920 & 357.389587 & 68.545930 & 15.229 & -23.45 & 3.21  & 1.071 & 0.867 & Gaia \\
    231   & King 11 & 23    & Gaia DR3 2211215057097380736 & 357.019110 & 68.544032 & 14.423 & -29.01 & 2.07  & 1.005 & 0.996 & Gaia \\
    232   & King 11 & 24    & Gaia DR3 2211216117949545216 & 356.988743 & 68.595175 & 11.656 & -22.53 & 0.83  & 1.103 & 0.999 & Gaia \\
    233   & King 11 & 25    & Gaia DR3 2211216190968724352 & 357.083832 & 68.615340 & 15.109 & -27.03 & 3.58  & 1.062 & 0.999 & Gaia \\
    234   & King 11 & 26    & Gaia DR3 2211216259688195840 & 357.083180 & 68.624853 & 13.538 & -24.27 & 0.65  & 1.138 & 0.999 & Gaia \\
    235   & King 11 & 27    & Gaia DR3 2211216259688197248 & 357.073903 & 68.619669 & 13.258 & -24.92 & 0.58  & 0.976 & 0.999 & Gaia \\
    236   & King 11 & 28    & Gaia DR3 2211216637645318016 & 357.107367 & 68.628733 & 15.211 & -27.27 & 2.86  & 0.939 & 0.999 & Gaia \\
    237   & King 11 & 29    & Gaia DR3 2211216809444343424 & 357.255762 & 68.666917 & 15.141 & -21.46 & 4.32  & 1.156 & 0.995 & Gaia \\
    238   & King 11 & 30    & Gaia DR3 2211218149473799680 & 357.402808 & 68.682865 & 14.535 & -23.97 & 1.94  & 1.014 & 0.986 & Gaia \\
    239   & King 11 & 31    & Gaia DR3 2211218218193278848 & 357.330836 & 68.669865 & 15.110 & -21.83 & 4.85  & 1.051 & 0.993 & Gaia \\
    240   & King 11 & 32    & Gaia DR3 2211218248254555392 & 357.334862 & 68.672016 & 14.950 & -36.70 & 7.28  & 1.025 & 0.994 & Gaia \\
    241   & King 11 & 33    & Gaia DR3 2211219111546472320 & 356.919877 & 68.608428 & 13.205 & -23.46 & 0.50  & 1.033 & 0.999 & Gaia \\
    242   & King 11 & 34    & Gaia DR3 2211219111546474368 & 356.931441 & 68.607349 & 14.964 & -25.73 & 3.39  & 0.992 & 1.000 & Gaia \\
    243   & King 11 & 35    & Gaia DR3 2211219145906206976 & 356.991901 & 68.627327 & 15.138 & -27.19 & 3.93  & 1.026 & 1.000 & Gaia \\
    244   & King 11 & 36    & Gaia DR3 2211219180265953280 & 357.007091 & 68.618011 & 15.073 & -30.24 & 3.80  & 0.987 & 0.999 & Gaia \\
    245   & King 11 & 37    & Gaia DR3 2211219248985423104 & 357.026281 & 68.630739 & 14.317 & -24.37 & 1.97  & 1.021 & 0.999 & Gaia \\
    246   & King 11 & 38    & Gaia DR3 2211219352064634752 & 356.965344 & 68.628259 & 14.983 & -21.38 & 2.77  & 1.290 & 0.999 & Gaia \\
    247   & King 11 & 39    & Gaia DR3 2211219352064975232 & 356.998063 & 68.640050 & 15.297 & -28.60 & 7.67  & 0.971 & 0.999 & Gaia \\
    248   & King 11 & 40    & Gaia DR3 2211219416485185792 & 356.953847 & 68.641161 & 15.433 & -42.17 & 5.57  & 0.961 & 1.000 & Gaia \\
    249   & King 11 & 41    & Gaia DR3 2211219455143847680 & 357.009210 & 68.636977 & 14.197 & -29.26 & 1.67  & 1.036 & 0.999 & Gaia \\
    250   & King 11 & 42    & Gaia DR3 2211220142338603776 & 356.926025 & 68.647576 & 15.037 & -21.55 & 3.89  & 1.049 & 1.000 & Gaia \\
    251   & King 11 & 43    & Gaia DR3 2211220142338605696 & 356.936266 & 68.645285 & 15.439 & -23.07 & 5.90  & 1.243 & 0.999 & Gaia \\
    252   & King 11 & 44    & Gaia DR3 2211220176698343168 & 356.949991 & 68.648796 & 13.798 & -26.48 & 1.37  & 1.081 & 0.999 & Gaia \\
    253   & King 11 & 45    & Gaia DR3 2211220211058075776 & 356.910835 & 68.656766 & 12.245 & -23.69 & 0.33  & 0.956 & 1.000 & Gaia \\
    254   & King 11 & 46    & Gaia DR3 2211220211058078080 & 356.947807 & 68.659669 & 15.052 & -22.19 & 4.39  & 1.030 & 1.000 & Gaia \\
    255   & King 11 & 47    & Gaia DR3 2211220348497025792 & 357.001815 & 68.680965 & 15.642 & -33.83 & 14.48 & 1.039 & 0.999 & Gaia \\
    256   & King 11 & 48    & Gaia DR3 2211220417216500096 & 356.929233 & 68.674805 & 15.096 & -27.60 & 3.05  & 1.065 & 0.999 & Gaia \\
    257   & King 11 & 49    & Gaia DR3 2211220451576239616 & 356.971568 & 68.679689 & 15.512 & -29.69 & 6.33  & 0.936 & 0.999 & Gaia \\
    258   & King 11 & 50    & Gaia DR3 2211220520295709952 & 356.947294 & 68.691200 & 15.401 & -27.33 & 5.46  & 1.021 & 0.999 & Gaia \\
    259   & King 11 & 51    & Gaia DR3 2211220520296057600 & 356.947975 & 68.681533 & 14.944 & -25.90 & 3.30  & 0.985 & 0.999 & Gaia \\
    260   & King 11 & 52    & Gaia DR3 2211220554655455488 & 357.008043 & 68.682825 & 14.945 & -22.62 & 4.06  & 1.014 & 0.998 & Gaia \\
    261   & King 11 & 53    & Gaia DR3 2214128277574911488 & 356.461782 & 68.665602 & 12.685 & -24.81 & 0.30  & 1.061 & 0.969 & Gaia \\
    262   & King 11 & 54    & Gaia DR3 2214128384954802176 & 356.599434 & 68.607619 & 15.190 & -27.34 & 5.26  & 1.078 & 0.996 & Gaia \\
    263   & King 11 & 55    & Gaia DR3 2214128552452820096 & 356.633619 & 68.627339 & 15.022 & -23.60 & 4.01  & 0.971 & 0.997 & Gaia \\
    264   & King 11 & 56    & Gaia DR3 2214128900350873600 & 356.732146 & 68.642600 & 15.059 & -21.24 & 4.00  & 1.037 & 0.999 & Gaia \\
    265   & King 11 & 57    & Gaia DR3 2214129037789819392 & 356.843432 & 68.675385 & 15.029 & -29.81 & 3.73  & 0.989 & 0.999 & Gaia \\
    266   & King 11 & 58    & Gaia DR3 2214129072149561216 & 356.865956 & 68.672727 & 15.572 & -10.77 & 4.83  & 0.986 & 0.999 & Gaia \\
    267   & King 11 & 59    & Gaia DR3 2214129278307970048 & 356.786459 & 68.699527 & 13.835 & -22.40 & 1.25  & 1.073 & 0.994 & Gaia \\
    268   & King 11 & 60    & Gaia DR3 2214129381387185664 & 356.815634 & 68.703584 & 13.536 & -114.17 & 0.58  & 1.052 & 0.999 & Gaia \\
    269   & King 11 & 61    & Gaia DR3 2214129828063769088 & 356.600136 & 68.697239 & 15.491 & -21.79 & 5.18  & 1.095 & 0.993 & Gaia \\
    270   & King 11 & 62    & Gaia DR3 2214129999862477184 & 356.716747 & 68.685504 & 15.585 & -15.34 & 6.01  & 1.034 & 0.998 & Gaia \\
    271   & King 11 & 63    & Gaia DR3 2214130102941681664 & 356.764024 & 68.713067 & 15.278 & -25.30 & 4.70  & 1.003 & 0.998 & Gaia \\
    272   & King 11 & 64    & Gaia DR3 2214130240380634624 & 356.857544 & 68.729733 & 15.076 & -25.80 & 3.00  & 1.056 & 0.998 & Gaia \\
    273   & King 11 & 65    & Gaia DR3 2214132783001262848 & 356.562127 & 68.701184 & 15.083 & -23.12 & 4.00  & 1.059 & 0.990 & Gaia \\
    274   & King 11 & 66    & Gaia DR3 2214222942953801600 & 356.962011 & 68.698777 & 14.964 & -26.67 & 3.52  & 1.015 & 0.999 & Gaia \\
    275   & King 11 & 67    & Gaia DR3 2214223011673276288 & 356.972348 & 68.717454 & 14.900 & 36.85 & 8.67  & 1.019 & 0.998 & Gaia \\
    276   & King 11 & 68    & Gaia DR3 2214223183472302464 & 356.913333 & 68.708479 & 15.168 & -23.25 & 4.27  & 1.024 & 0.999 & Gaia \\
    277   & King 11 & 69    & Gaia DR3 2214227375360032512 & 356.903357 & 68.794866 & 14.683 & -19.40 & 2.90  & 1.030 & 0.991 & Gaia \\
    278   & King 12 & 1     & Gaia DR3 2012765337282245888 & 358.070257 & 61.877564 & 7.022 & -41.25 & 0.30  & 0.912 & 0.780 & Gaia \\
    279   & King 12 & 2     & Gaia DR3 2012771861325524992 & 358.273640 & 61.951561 & 10.272 & -64.29 & 19.80 & 0.821 & 0.996 & Gaia \\
    280   & King 13 & 1     & Gaia DR3 429243193398029696 & 2.770341 & 60.984203 & 13.675 & -58.59 & 1.20  & 0.967 & 0.525 & Gaia \\
    281   & King 13 & 2     & Gaia DR3 429247660163942784 & 2.477626 & 61.078925 & 13.900 & -59.59 & 1.89  & 0.987 & 0.996 & Gaia \\
    282   & King 13 & 3     & Gaia DR3 429608987172405248 & 2.948175 & 61.086618 & 14.137 & -60.20 & 1.64  & 1.057 & 0.725 & Gaia \\
    283   & King 13 & 4     & Gaia DR3 429620910001551744 & 2.604855 & 61.171808 & 13.928 & -57.14 & 1.86  & 1.093 & 0.997 & Gaia \\
    284   & King 13 & 5     & Gaia DR3 429620944361277184 & 2.597658 & 61.185180 & 13.624 & -61.30 & 1.88  & 1.023 & 0.998 & Gaia \\
    285   & King 13 & 6     & Gaia DR3 429621494117117440 & 2.760588 & 61.180403 & 14.018 & -57.25 & 1.69  & 1.013 & 0.997 & Gaia \\
    286   & King 13 & 7     & Gaia DR3 429622112592408704 & 2.720099 & 61.171996 & 14.040 & -58.88 & 1.52  & 1.065 & 0.956 & Gaia \\
    287   & King 13 & 8     & Gaia DR3 429623624420879488 & 2.514501 & 61.160173 & 13.646 & -58.07 & 1.86  & 1.041 & 0.996 & Gaia \\
    288   & King 13 & 9     & Gaia DR3 429623796219563264 & 2.530681 & 61.172401 & 14.088 & -59.69 & 2.92  & 1.130 & 0.996 & Gaia \\
    289   & King 13 & 10    & Gaia DR3 429623963714693376 & 2.538714 & 61.205225 & 12.337 & -66.12 & 3.73  & 1.219 & 0.989 & Gaia \\
    290   & King 13 & 11    & Gaia DR3 429624036737717632 & 2.513526 & 61.184330 & 13.944 & -60.88 & 2.90  & 1.039 & 0.939 & Gaia \\
    291   & King 13 & 12    & Gaia DR3 429624208536368384 & 2.461783 & 61.222005 & 13.975 & -60.02 & 1.81  & 1.084 & 0.998 & Gaia \\
    292   & King 13 & 13    & Gaia DR3 429624827011668096 & 2.429507 & 61.204577 & 14.048 & -59.66 & 1.89  & 0.988 & 0.997 & Gaia \\
    293   & King 13 & 14    & Gaia DR3 429625376767501440 & 2.567292 & 61.207461 & 14.005 & -59.85 & 2.77  & 1.068 & 0.997 & Gaia \\
    294   & King 13 & 15    & Gaia DR3 429625582925904256 & 2.553293 & 61.235582 & 13.979 & -57.69 & 2.08  & 0.975 & 0.996 & Gaia \\
    295   & King 14 & 1     & Gaia DR3 430973652900383232 & 7.294182 & 63.118286 & 8.953 & -54.82 & 0.17  & 0.978 & 0.950 & Gaia \\
    296   & King 15 & 1     & Gaia DR3 430267457196171264 & 8.290008 & 61.835830 & 12.706 & -65.01 & 0.53  & 0.973 & 0.857 & Gaia \\
    297   & King 15 & 2     & Gaia DR3 430268861642658176 & 8.312254 & 61.841222 & 13.090 & -69.50 & 2.44  & 1.150 & 0.985 & Gaia \\
    298   & King 15 & 3     & Gaia DR3 430268900305177088 & 8.309797 & 61.857466 & 12.210 & -66.95 & 0.42  & 0.988 & 0.704 & Gaia \\
    299   & King 15 & 4     & Gaia DR3 430316419827197440 & 8.266902 & 61.905115 & 14.217 & -7.75 & 6.94  & 1.033 & 0.774 & Gaia \\
    300   & King 15 & 5     & Gaia DR3 430267457196171264 & 8.289987 & 61.835825 & 12.721 & -64.69 & 0.06  & 0.973 & 0.857 & APOGEE \\
    301   & King 16 & 1     & Gaia DR3 523960107175429632 & 10.714451 & 64.034616 & 9.193 & -46.49 & 0.30  & 0.908 & 0.973 & Gaia \\
    302   & King 17 & 1     & Gaia DR3 188467150678936960 & 77.165796 & 39.028554 & 15.792 & -2.56 & 3.48  & 1.095 & 0.787 & LAMOST \\
    303   & King 18 & 1     & Gaia DR3 2007391302402423424 & 343.058320 & 58.289435 & 12.223 & -63.10 & 0.33  & 0.957 & 0.993 & Gaia \\
    304   & King 18 & 2     & Gaia DR3 2007402709835538944 & 343.004673 & 58.292232 & 11.938 & -62.43 & 0.38  & 0.944 & 0.986 & Gaia \\
    305   & King 18 & 3     & Gaia DR3 2007402877328867328 & 342.973274 & 58.302970 & 12.456 & 84.40 & 10.15 & 0.960 & 0.987 & Gaia \\
    306   & King 18 & 4     & Gaia DR3 2007403220926248576 & 343.078322 & 58.335212 & 11.749 & -61.65 & 0.34  & 0.832 & 0.991 & Gaia \\
    307   & King 18 & 5     & Gaia DR3 2013397315944192384 & 343.488141 & 58.396855 & 11.587 & -45.08 & 0.28  & 0.897 & 0.663 & Gaia \\
    308   & King 19 & 1     & Gaia DR3 2014044103657399040 & 346.886679 & 60.411860 & -44.760 & 0.39  & 1.13  & 1.126 & 0.989 & Gaia \\
    309   & King 19 & 2     & Gaia DR3 2014045787284525056 & 347.024505 & 60.517559 & -41.520 & 3.09  & 1.12  & 1.115 & 0.999 & Gaia \\
    310   & King 19 & 3     & Gaia DR3 2014048742223801600 & 347.005428 & 60.523482 & -61.740 & 1.33  & 1.22  & 1.215 & 0.999 & Gaia \\
    311   & King 19 & 4     & Gaia DR3 2014051319202432128 & 347.060299 & 60.494636 & -60.230 & 2.48  & 0.96  & 0.956 & 0.987 & Gaia \\
    312   & King 19 & 5     & Gaia DR3 2014051456641382656 & 347.123074 & 60.518700 & -54.660 & 2.96  & 1.09  & 1.087 & 0.999 & Gaia \\
    313   & King 19 & 6     & Gaia DR3 2014051589783371648 & 347.035725 & 60.520152 & -49.870 & 16.91 & 1.33  & 1.332 & 0.995 & Gaia \\
    314   & King 19 & 7     & Gaia DR3 2014051624137262208 & 347.065309 & 60.523590 & -62.780 & 2.09  & 0.98  & 0.981 & 0.998 & Gaia \\
    315   & King 19 & 8     & Gaia DR3 2014051628440053376 & 347.089942 & 60.533316 & -60.360 & 2.13  & 1.07  & 1.071 & 0.999 & Gaia \\
    316   & King 19 & 9     & Gaia DR3 2014051662799786752 & 347.037433 & 60.521198 & -60.070 & 1.48  & 1.04  & 1.040 & 0.997 & Gaia \\
    317   & King 19 & 10    & Gaia DR3 2014051972037720960 & 347.202224 & 60.558309 & -60.710 & 1.77  & 0.98  & 0.979 & 0.998 & Gaia \\
    318   & King 19 & 11    & Gaia DR3 2014052143836118912 & 347.154456 & 60.565443 & -61.870 & 1.29  & 1.07  & 1.072 & 0.998 & Gaia \\
    319   & King 19 & 12    & Gaia DR3 2014054892615156096 & 347.015094 & 60.556700 & -62.300 & 0.71  & 0.96  & 0.963 & 0.999 & Gaia \\
    320   & King 21 & 1     & Gaia DR3 2015970619831662464 & 357.473870 & 62.683290 & 13.569 & -30.02 & 3.54  & 0.978 & 0.998 & APOGEE \\
    321   & King 21 & 2     & Gaia DR3 2015970722910762624 & 357.512371 & 62.700872 & 13.492 & -45.37 & 2.86  & 1.013 & 0.999 & APOGEE \\
    322   & King 21 & 3     & Gaia DR3 2015971753702889088 & 357.496202 & 62.722331 & 13.143 & -31.80 & 0.49  & 1.161 & 0.999 & APOGEE \\
    323   & King 22 & 1     & Gaia DR3 208501425066639360 & 80.913034 & 45.322760 & 14.802 & -21.33 & 3.21  & 1.054 & 0.835 & Gaia \\
    324   & King 22 & 2     & Gaia DR3 208535475567047040 & 80.001543 & 45.266420 & 14.461 & -34.79 & 9.49  & 0.983 & 0.516 & Gaia \\
    325   & King 22 & 3     & Gaia DR3 208538567943466880 & 80.404469 & 45.103443 & 15.020 & 0.43  & 5.16  & 0.999 & 0.701 & Gaia \\
    326   & King 22 & 4     & Gaia DR3 208541900838022912 & 80.501818 & 45.231961 & 14.736 & 1.58  & 2.42  & 1.062 & 0.977 & Gaia \\
    327   & King 22 & 5     & Gaia DR3 208546436323442560 & 80.525293 & 45.349606 & 14.502 & -2.55 & 2.22  & 1.037 & 0.997 & Gaia \\
    328   & King 22 & 6     & Gaia DR3 208551315406283136 & 80.564078 & 45.342294 & 13.664 & -2.73 & 0.53  & 1.152 & 0.994 & Gaia \\
    329   & King 22 & 7     & Gaia DR3 208551899521782656 & 80.669345 & 45.393576 & 13.561 & -2.71 & 0.98  & 1.014 & 0.997 & Gaia \\
    330   & King 22 & 8     & Gaia DR3 208552208759461632 & 80.600549 & 45.367262 & 14.508 & -0.61 & 2.39  & 1.075 & 0.998 & Gaia \\
    331   & King 22 & 9     & Gaia DR3 208552243119185280 & 80.618714 & 45.388153 & 14.265 & -2.87 & 1.96  & 1.072 & 0.998 & Gaia \\
    332   & King 22 & 10    & Gaia DR3 208552449277627136 & 80.571306 & 45.394728 & 15.017 & -3.54 & 4.81  & 1.006 & 0.999 & Gaia \\
    333   & King 22 & 11    & Gaia DR3 208552483637350144 & 80.608756 & 45.403354 & 15.343 & -2.31 & 5.31  & 1.067 & 0.998 & Gaia \\
    334   & King 22 & 12    & Gaia DR3 208552689795761920 & 80.654026 & 45.411054 & 15.170 & -4.74 & 4.35  & 0.955 & 0.998 & Gaia \\
    335   & King 22 & 13    & Gaia DR3 208554545223660672 & 80.737684 & 45.485238 & 15.034 & -1.03 & 5.07  & 1.011 & 0.993 & Gaia \\
    336   & King 22 & 14    & Gaia DR3 208558152994233600 & 80.487669 & 45.356111 & 15.228 & -0.84 & 5.31  & 1.036 & 0.998 & Gaia \\
    337   & King 22 & 15    & Gaia DR3 208558221713704064 & 80.482404 & 45.376336 & 14.853 & -16.42 & 4.05  & 0.984 & 0.561 & Gaia \\
    338   & King 22 & 16    & Gaia DR3 208558634030530816 & 80.530891 & 45.427438 & 14.968 & -10.19 & 4.53  & 1.017 & 0.999 & Gaia \\
    339   & King 22 & 17    & Gaia DR3 208559493024828544 & 80.455303 & 45.422939 & 15.085 & -14.32 & 5.03  & 1.015 & 0.998 & Gaia \\
    340   & King 22 & 18    & Gaia DR3 208559527384566656 & 80.478172 & 45.439623 & 13.905 & -4.95 & 1.38  & 1.049 & 0.999 & Gaia \\
    341   & King 22 & 19    & Gaia DR3 208559591805552768 & 80.475559 & 45.445223 & 15.143 & -10.87 & 5.96  & 0.944 & 0.999 & Gaia \\
    342   & King 22 & 20    & Gaia DR3 208559729244006784 & 80.527565 & 45.478580 & 15.245 & 7.49  & 5.87  & 0.997 & 0.998 & Gaia \\
    343   & King 22 & 21    & Gaia DR3 208560455096736256 & 80.320155 & 45.369758 & 13.869 & -2.82 & 1.38  & 1.070 & 0.988 & Gaia \\
    344   & King 22 & 22    & Gaia DR3 208561966925206912 & 80.363552 & 45.397653 & 14.975 & 5.24  & 6.56  & 0.948 & 0.995 & Gaia \\
    345   & King 22 & 23    & Gaia DR3 208562374944879360 & 80.402670 & 45.444996 & 14.946 & -67.90 & 3.32  & 1.107 & 0.837 & Gaia \\
    346   & King 22 & 24    & Gaia DR3 208562791558872192 & 80.452792 & 45.482297 & 14.227 & -2.35 & 1.73  & 1.132 & 0.998 & Gaia \\
    347   & King 22 & 25    & Gaia DR3 208563856710716800 & 80.494641 & 45.551654 & 15.152 & 1.16  & 4.71  & 0.966 & 0.997 & Gaia \\
    348   & King 22 & 26    & Gaia DR3 208564269027610880 & 80.578109 & 45.421975 & 15.028 & 3.62  & 4.46  & 1.063 & 0.999 & Gaia \\
    349   & King 22 & 27    & Gaia DR3 208564402168390272 & 80.619943 & 45.456913 & 13.550 & -1.46 & 0.84  & 0.995 & 0.999 & Gaia \\
    350   & King 22 & 28    & Gaia DR3 208564406466538240 & 80.624207 & 45.448703 & 14.594 & -4.36 & 2.77  & 1.081 & 0.998 & Gaia \\
    351   & King 22 & 29    & Gaia DR3 208564543905510656 & 80.559430 & 45.450009 & 14.935 & -2.68 & 3.45  & 0.941 & 0.997 & Gaia \\
    352   & King 22 & 30    & Gaia DR3 208564715704170112 & 80.648596 & 45.458661 & 14.431 & -2.47 & 2.11  & 1.002 & 0.998 & Gaia \\
    353   & King 22 & 31    & Gaia DR3 208565368539223936 & 80.557622 & 45.466363 & 15.073 & -3.52 & 3.99  & 1.001 & 0.998 & Gaia \\
    354   & King 22 & 32    & Gaia DR3 208565540337913984 & 80.544407 & 45.480383 & 14.308 & -1.60 & 2.00  & 1.005 & 0.999 & Gaia \\
    355   & King 22 & 33    & Gaia DR3 208565677776849024 & 80.580004 & 45.495889 & 13.402 & -0.66 & 0.45  & 1.036 & 0.998 & Gaia \\
    356   & King 22 & 34    & Gaia DR3 208568735793543296 & 80.590192 & 45.533047 & 15.422 & 7.85  & 5.34  & 0.984 & 0.997 & Gaia \\
    357   & King 22 & 35    & Gaia DR3 208725725438582528 & 80.130129 & 45.420640 & 14.571 & -28.69 & 3.82  & 1.028 & 0.908 & Gaia \\
    358   & King 22 & 36    & Gaia DR3 208750773687826304 & 80.319627 & 45.554739 & 13.722 & -5.91 & 1.41  & 1.024 & 0.965 & Gaia \\
    359   & King 22 & 37    & Gaia DR3 208759702920764032 & 80.593595 & 45.746941 & 14.959 & -48.61 & 5.40  & 1.001 & 0.839 & Gaia \\
    360   & King 22 & 38    & Gaia DR3 208764655022061184 & 80.679138 & 45.839181 & 13.273 & -15.13 & 0.87  & 1.127 & 0.607 & Gaia \\
    361   & King 22 & 39    & Gaia DR3 208562791558872192 & 80.452797 & 45.482296 & 14.248 & -0.82 & 1.77  & 1.132 & 0.998 & LAMOST \\
    362   & King 23 & 1     & Gaia DR3 3109982902759582336 & 110.428060 & -1.093076 & 14.353 & -13.44 & 8.04  & 1.103 & 0.996 & Gaia \\
    363   & King 23 & 2     & Gaia DR3 3109986063855413120 & 110.452229 & -0.992237 & 13.118 & 53.09 & 1.32  & 1.004 & 0.998 & Gaia \\
    364   & King 23 & 3     & Gaia DR3 3109986166934612352 & 110.469199 & -0.987512 & 13.247 & 56.44 & 1.50  & 1.039 & 0.998 & Gaia \\
    365   & King 23 & 4     & Gaia DR3 3109986166934620928 & 110.468140 & -0.994460 & 11.822 & 35.14 & 10.55 & 0.958 & 0.998 & Gaia \\
    366   & King 23 & 5     & Gaia DR3 3109988675195552128 & 110.419775 & -0.995129 & 14.209 & 31.34 & 9.63  & 1.115 & 0.998 & Gaia \\
    367   & King 23 & 6     & Gaia DR3 3109989121872110080 & 110.464423 & -0.981849 & 12.373 & 53.44 & 0.66  & 1.032 & 0.891 & Gaia \\
    368   & King 23 & 7     & Gaia DR3 3109989362390291840 & 110.417194 & -0.958622 & 14.070 & 49.11 & 3.54  & 1.013 & 0.944 & Gaia \\
    369   & King 23 & 8     & Gaia DR3 3109989392447848960 & 110.440530 & -0.960476 & 12.263 & 53.30 & 0.46  & 1.012 & 0.997 & Gaia \\
    370   & King 23 & 9     & Gaia DR3 3109989396744298624 & 110.428063 & -0.963390 & 12.123 & 55.39 & 0.48  & 0.896 & 0.973 & Gaia \\
    371   & King 23 & 10    & Gaia DR3 3109989843425908608 & 110.333486 & -0.974640 & 14.108 & 49.02 & 9.39  & 1.018 & 0.994 & Gaia \\
    372   & King 23 & 11    & Gaia DR3 3109995718941761536 & 110.546661 & -0.898627 & 11.293 & 53.65 & 0.23  & 1.305 & 0.994 & Gaia \\
    373   & King 23 & 12    & Gaia DR3 3109990942939026304 & 110.551333 & -1.012381 & 14.617 & 61.16 & 3.17  & 0.923 & 0.996 & LAMOST \\
    374   & King 23 & 13    & Gaia DR3 3109986166934612352 & 110.469197 & -0.987515 & 13.258 & 56.31 & 1.13  & 1.039 & 0.998 & LAMOST \\
    375   & King 23 & 14    & Gaia DR3 3109989121872110080 & 110.464420 & -0.981852 & 12.384 & 53.74 & 0.61  & 1.032 & 0.891 & LAMOST \\
    376   & King 24 & 1     & Gaia DR3 5598737814515190528 & 117.597923 & -29.938372 & 14.243 & 73.70 & 1.64  & 1.085 & 0.995 & Gaia \\
    377   & King 24 & 2     & Gaia DR3 5598738914026824192 & 117.561015 & -29.899669 & 13.678 & 72.45 & 0.96  & 1.074 & 0.994 & Gaia \\
    378   & King 24 & 3     & Gaia DR3 5598739120185245312 & 117.577696 & -29.893318 & 15.153 & 75.54 & 4.94  & 0.954 & 0.994 & Gaia \\
    379   & King 24 & 4     & Gaia DR3 5598739154544972160 & 117.592193 & -29.881553 & 15.341 & 74.23 & 4.14  & 1.019 & 0.998 & Gaia \\
    380   & King 24 & 5     & Gaia DR3 5598739188904698752 & 117.613180 & -29.880552 & 14.557 & 74.14 & 2.12  & 1.047 & 0.998 & Gaia \\
    381   & King 24 & 6     & Gaia DR3 5598739291983898368 & 117.622968 & -29.858023 & 14.640 & 75.86 & 4.66  & 0.990 & 0.998 & Gaia \\
    382   & King 24 & 7     & Gaia DR3 5598739566861808128 & 117.603232 & -29.834368 & 14.809 & 70.78 & 2.61  & 1.016 & 0.998 & Gaia \\
    383   & King 24 & 8     & Gaia DR3 5598743999268318592 & 117.689148 & -29.899657 & 15.382 & 55.30 & 3.91  & 0.971 & 0.968 & Gaia \\
    384   & King 24 & 9     & Gaia DR3 5598744342865424768 & 117.649999 & -29.869743 & 14.283 & 74.26 & 1.74  & 1.009 & 0.996 & Gaia \\
    385   & King 24 & 10    & Gaia DR3 5598744892621203200 & 117.701546 & -29.833480 & 14.459 & 72.96 & 3.17  & 1.032 & 0.994 & Gaia \\
    386   & King 24 & 11    & Gaia DR3 5598745167499148928 & 117.630751 & -29.847578 & 13.280 & 74.38 & 0.56  & 1.013 & 0.998 & Gaia \\
    387   & King 24 & 12    & Gaia DR3 5598745236218607104 & 117.664490 & -29.844956 & 15.154 & 73.50 & 3.56  & 1.019 & 0.997 & Gaia \\
    388   & King 24 & 13    & Gaia DR3 5598745304938086656 & 117.653668 & -29.836302 & 15.107 & 71.68 & 5.20  & 1.101 & 0.997 & Gaia \\
    389   & King 24 & 14    & Gaia DR3 5598745408017307008 & 117.638508 & -29.828798 & 14.732 & 73.46 & 2.66  & 1.019 & 0.997 & Gaia \\
    390   & King 24 & 15    & Gaia DR3 5598745476736789120 & 117.622783 & -29.822137 & 15.408 & 69.38 & 3.65  & 1.030 & 0.985 & Gaia \\
    391   & King 24 & 16    & Gaia DR3 5598786811503789824 & 117.544900 & -29.809212 & 15.157 & 75.13 & 3.09  & 1.014 & 0.995 & Gaia \\
    392   & King 25 & 1     & Gaia DR3 4319541488271342848 & 291.089871 & 13.581142 & 12.931 & 11.96 & 0.37  & 1.015 & 0.987 & Gaia \\
    393   & King 25 & 2     & Gaia DR3 4319542239879768576 & 291.125379 & 13.636344 & 12.516 & 14.36 & 0.24  & 0.968 & 0.987 & Gaia \\
    394   & King 25 & 3     & Gaia DR3 4319544065252007808 & 291.165782 & 13.686341 & 13.037 & 11.47 & 0.37  & 1.069 & 0.993 & Gaia \\
    395   & King 25 & 4     & Gaia DR3 4319569079142236672 & 291.230623 & 13.780781 & 14.925 & 66.68 & 10.28 & 0.991 & 0.986 & Gaia \\
    396   & King 25 & 5     & Gaia DR3 4319569457099349248 & 291.279864 & 13.807278 & 14.751 & 137.12 & 7.20  & 0.995 & 0.913 & Gaia \\
    397   & King 26 & 1     & Gaia DR3 4321226455483980544 & 292.269639 & 14.766872 & 12.399 & 24.80 & 0.53  & 0.868 & 0.991 & Gaia \\
    398   & King 27 & 1     & Gaia DR3 1825883819833710848 & 295.523906 & 20.856738 & 13.340 & 18.56 & 0.49  & 1.022 & 0.797 & Gaia \\
    399   & King 27 & 2     & Gaia DR3 1825916869572580224 & 295.776278 & 21.106426 & 14.546 & 7.95  & 11.57 & 0.947 & 0.726 & Gaia \\
    400   & King 27 & 3     & Gaia DR3 1826099392812290944 & 295.416215 & 21.274312 & 12.396 & 27.49 & 0.19  & 0.868 & 0.603 & Gaia \\   
    401   & King 27 & 4     & Gaia DR3 1826105371408470528 & 295.655623 & 21.140130 & 13.414 & 17.67 & 1.02  & 1.008 & 0.845 & Gaia \\
    402   & King 27 & 5     & Gaia DR3 1826105745051312000 & 295.665319 & 21.153945 & 14.527 & 104.42 & 9.67  & 1.010 & 0.546 & Gaia \\
    403   & King 27 & 6     & Gaia DR3 1826105852444845056 & 295.663125 & 21.176461 & 12.851 & 17.34 & 2.79  & 0.961 & 0.699 & Gaia \\ 
    \hline
    \end{tabular}%
  \end{table*}%

